Two-Sided Weak Submodularity for Matroid Constrained Optimization and Regression

We study the following problem: Given a variable of interest, we would like to find a best linear predictor for it by choosing a subset of $k$ relevant variables obeying a matroid constraint. This problem is a natural generalization of subset selection problems where it is necessary to spread observations amongst multiple different classes. We derive new, strengthened guarantees for this problem by improving the analysis of the residual random greedy algorithm and by developing a novel distorted local-search algorithm. To quantify our approximation guarantees, we refine the definition of weak submodularity by Das and Kempe and introduce the notion of an upper submodularity ratio, which we connect to the minimum $k$-sparse eigenvalue of the covariance matrix. More generally, we look at the problem of maximizing a set function $f$ with lower and upper submodularity ratio $\gamma$ and $\beta$ under a matroid constraint. For this problem, our algorithms have asymptotic approximation guarantee $1/2$ and $1-e^{-1}$ as the function is closer to being submodular. As a second application, we show that the Bayesian A-optimal design objective falls into our framework, leading to new guarantees for this problem as well.

==> local-search.tex <==
\section{Local-Search}
\label{sec:bound-qual-local}
In this section, we derive a first novel algorithm to optimize $(\gamma, \beta)$-weakly submodular functions.
The algorithm is a simple local-search procedure. It exchanges elements as long it yields an improvement in the objective function. Each exchange preserves the feasibility of the set. To ensure a convergence in polynomial time, the algorithm performs the exchange only if the objective value increases by a $(1 + \e/k)$-multiplicative factor , and terminates after making at most $\lceil\log_{1+\e/k}k\rceil$ improvements. In order to ensure that a good solution is obtained after at most this number of improvements, we require a good starting solution. Here, we take the single element $e \in X$ with largest value $f(e)$, and complete $\{e\}$ arbitrarily to a base of $\cM$.
\begin{algorithm}[t]
    \SetKwProg{myproc}{procedure}{}{}
    \myproc{$\textsc{LocalSearch}(\cM, f, \e)$}{
      Let $e_{\mathrm{max}} = \argmax_{e \in X} f(e)$\;
      $S \gets $ an arbitrary base of $\cM$ containing $e_{\mathrm{max}}$\;
        \For{$i \gets 1$ \KwTo $\lceil\log_{1+\e/k} k \rceil$}{
           \uIf{$\exists e \in S$ and $e' \in X\bb S$ with $S - e + e' \in \cI$ and $(1 + \e/k)f(S) < f(S - e + e')$}{
             $S \gets S - e + e'$
           }
           \lElse{\Return{$S$}}
         }
         \Return{$S$}\;
    }
    \caption{The local-search algorithm}
    \label{alg:local-search}
\end{algorithm}



The next lemma gives the guarantees of the algorithm \ref{alg:local-search} for maximizing a $(\gamma, \beta)$-weakly submodular function.
Motivated by the $R^2$ objective (see section \ref{sec:R2}), for $(\gamma, 1/\gamma)$-weakly submodular function and assuming $\e = 0$, we recover a $1/2$-approximation as expected. The guarantee is also larger than $(1 + 1/\gamma)^{-2}$ for all $\gamma > \frac{\sqrt{5}-1}{2}$ and sufficiently small $\epsilon$.
\begin{theorem}
    Given a matroid $\cM = (X, \cI)$, a $(\gamma, \beta)$-weakly submodular function $f$ and $\e > 0$, the local-search algorithm \ref{alg:local-search} runs in time $\cO(nk^2\log(k)/\e)$ and returns a solution $S$ such that
$f(S) \geq \frac{\gamma^2}{(2-\gamma)\beta + \gamma^2 + \e} f(O)$ for any solution $O \in \cI$.
    \label{lem:loc-search-approx}
\end{theorem}
%This is the first polynomial-time algorithm that uses $\beta$-weak submodularity to derive an approximation that can beat Chen et al.'s algorithm \cite{Chen:2018:Weakly}.


% We now suppose that $f$ is $(\gamma, \beta)$-weakly submodular and consider a local optimum $S$ for the 1-local search procedure.
%In order to derive our guarantee, we make use of the following result.
\begin{proof}
Let $S_{\textrm{init}}$ be the arbitrary base $\cM$ containing $\argmax_{e \in X}f(e)$ that we select at the start of the algorithm. Consider any feasible solution $O \in \cI$. Then, by monotonicity, normalization of $f$ and $\gamma$-weak submodularity of $f$, we have $f(O) \leq \frac{1}{\gamma}\sum_{o \in O} f(o | \emptyset) \leq \frac{k}{\gamma}f(e) \leq \frac{k}{\gamma}f(S_{\textrm{init}})$. Each time the algorithm makes an exchange the value of the solution $S$ increases by a factor $(1+\e/k)$. Thus, if the algorithm terminates after $\lceil \log_{1 + \e/k} k\rceil$ improvements, then $f(S) \geq k f(S_{\textrm{init}}) \geq \gamma f(O) \geq \frac{\gamma^2}{\gamma^2 + \beta(2 - \gamma) + \e}f(O)$ as required.

Suppose now that the algorithm returns $S$ before making $\lceil \log_{1+\e/k}k \rceil$ improvements. Let $S = \{s_1,\ldots,s_k\}$. Since $\cM$ is a matroid, we can index the elements $o_i \in O$ and $s_i \in S$ so that $S - s_i + o_i$ is a feasible set for all $1 \leq i \leq k$. Since the algorithm terminated without making any further improvements, $(1+\epsilon/k)f(S) \geq f(S - s_i + o_i)$ for all $1 \leq i \leq k$. Subtracting $f(S-s_i)$ from each side, and applying Lemma~\ref{lem:weak-marginals} gives:
    \begin{equation*}
        f(s_i | S-s_i) + (\epsilon/k) f(S) \geq f(o_i | S - s_i) \geq \gamma f(o_i|S) - (1-\gamma)f(s_i|S-s_i),
    \end{equation*}
for all $i \leq i \leq k$. Summing over all $i$ and rearranging we then have:
    \begin{equation*}
        (2 - \gamma)\sum_{i = 1}^kf(s_i | S-s_i) + \epsilon f(S) \geq \gamma \sum_{i = 1}^k f(o_i | S)\,.
    \end{equation*}
    Now, we use $\beta$-weak submodularity to upper-bound the left-hand side, and $\gamma$-weak submodularity and monotonicity of $f$ to lower-bound the right-hand side:
    \begin{equation*}
        ((2 - \gamma)\beta + \epsilon)f(S) \geq \gamma^2(f(O \cup S) - f(S)) \geq \gamma^2(f(O) - f(S))
    \end{equation*}
Rearranging this then gives the claimed guarantee.
    % \begin{equation*}
    %     \frac{(2 - \gamma)\beta + \gamma^2 + \epsilon}{\gamma^2}f(S) \geq f(O).
    % \end{equation*}
The bound on the running time follows from the fact that the algorithm makes at most $\lceil\log_{1+\e/k}k\rceil = O(k\log(k)/\e)$ improvements, each of which can be found in time $O(nk)$.
\end{proof}

% Observe that for when $\beta \leq \frac{1}{\gamma}$, similar to the $R^2$ objective function introduced in section \ref{sec:R2}, we get an approximation ratio of:
% $
%     \frac{\gamma^2}{\frac{2}{\gamma}-1+\gamma^2 + \epsilon}.
% $
% Note that when $\gamma = 1$, this is 1/2 as expected.
% It is also larger than $(1+1/\gamma)^{-2}$ for all $\gamma > 1/3$.
% Note that when $\gamma = 1$, and $\epsilon = 0$ this is 1/2 as expected. It is also larger than Chen et al.'s guarantee of $(1+1/\gamma)^{-2}$ \cite{Chen:2018:Weakly} for all $\gamma > \frac{\sqrt{5}-1}{2}$ and sufficiently small $\epsilon$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Submission"
%%% End:


==> preliminaries.tex <==
\section{Preliminaries}
\begin{itemize}
    \item def submodular
    \item def matroid
    \item generalized $\gamma$.
    \item goal
    \item standard notation
    \item Organization paper
    \item main results
    \item
\end{itemize}
In this section, we introduce the key definitions, results and notations that we will use throughout the paper.
A set function $f: 2^\mathcal{N}\rightarrow\RR$ is monotone if for any two sets $A\subseteq B \subseteq \mathcal{N}$: $f(A) \leq f(B)$. We say that $f$ is non-negative if $f(A) \geq 0$ for all $A \subseteq \mathcal{N}$.
Given a set $B$, we denote by $f(B \mid A) := f(B \cup A) - f(A)$ the marginal contribution of adding a set $B$ to $A$. For simplicity when $B = \{e\}$ is a singleton we ignore the brackets and we write $f(e \mid A)$ instead of $f(\{e\}\mid A)$. Moreover, we use $A+e$ and $A-e$ to define the union $A \cup \{e\}$ and removal $A \bb\{e\}$ of $e$.
The following definition refines the notion of weak submodularity. We introduce a new parameter $\beta_{\cU,k}$ which measures the loss by removing an entire set compared to the aggretate individual losses.
\begin{definition}
    Let $f:2^\mathcal{N} \rightarrow \RR_{\geq 0}$ be a set function. The lower submodularity ratio of $f$ with respect to $\cU$ and an integer $k$ is
    \begin{align*}
        \gamma_{\mathcal{U}, k} = \min_{\substack{S \subseteq \mathcal{U}, T \colon \card{T}\leq k, \\ S \cap T = \emptyset.}} \frac{\sum_{e \in T} f(S + e) - f(S)}{f(T \cup S) - f(S)}.
    \end{align*}
    The upper submodularity ratio of $f$ with respect to $\mathcal{U}$ and $k$ is
    \begin{align*}
        \beta_{\cU, k} = \max_{\substack{S \subseteq \cU, T \colon \card{T}\leq k, \\ S \cap T = \emptyset.}} \frac{\sum_{e \in T} f(S \cup T) - f(S \cup T - e)}{f(T \cup S) - f(S)}.
    \end{align*}
    \label{def:weak-submod}
\end{definition}
The ratio $\gamma_{\cU, k}$ was introduced by Das and Kempe \cite{DBLP:journals/jmlr/DasK18} to measure how close a set function is from being submodular. In particular, the ratio $\gamma_{\cU, k} \geq 1$ for all $\cU, k$ if and only if $f$ is submodular.
The new ratio $\beta_{U, k}$ has the same purpose but is incomparable with $\gamma_{\cU,k}$ in general. Similarly, the function $f$ is submodular if and only if $\beta_{\cU, k} \leq 1$.

\begin{definition}
    \label{def:matroid}
    A matroid $\cM = (X, \cI)$ is a pair where $X$ is a finite set of elements and $\cI$ is a family of subset such that
    \begin{itemize}
        \item if $ A \subseteq B \subseteq X$ and $B \in \cI$, then $A \in \cI$.
        \item if $A, B \in \cI$ and $\card{A} < \card{B}$, then there exists $e \in B \bb A$ such that $A + e \in \cI$.
    \end{itemize}
\end{definition}

\begin{definition}
    \label{def:weak-function}
    Given a set $\cU$ and an integer $k > 0$, we say that a set function $f: 2^\mathcal{N}\rightarrow\RR_{\geq 0}$ is a $(\gamma_{\cU, k}, \beta_{\cU, k})$-weakly submodular function, if the lower/upper weak submodularity ratio is greater than $\gamma_{\cU, k}$/lower than $\beta_{\cU, k}$, respecively.
\end{definition}
    When $\cU$ and $k$ are clear from the context, we will write $(\gamma, \beta)$ instead of $(\gamma_{\cU,k}, \beta_{\cU, k})$.
    \textbf{Notations:} Unless specified, we use the bold font $\vv$ to denote vectors and capital letters $A, B, \ldots$ to denote matrices. The $i^\textrm{th}$ coordinate of $\vv$ is denoted by $v_i$. We define $\hv_i$ as the vector $\vv$ with its $i^\textrm{th}$ coordinate removed, i.e., $\hv_i^T = (v_1, \ldots, v_{i-1}, v_{i+1}, \ldots, v_n)$. Similarly for a matrix $C$, we write $\hC_i$ as the matrix $C$ with the $i^\textrm{th}$ row and column removed.

